Graph Partitioning for Independent Sets

Computing maximum independent sets in graphs is an important problem in computer science. In this paper, we develop an evolutionary algorithm to tackle the problem. The core innovations of the algorithm are very natural combine operations based on graph partitioning and local search algorithms. More precisely, we employ a state-of-the-art graph partitioner to derive operations that enable us to quickly exchange whole blocks of given independent sets. To enhance newly computed offsprings we combine our operators with a local search algorithm. Our experimental evaluation indicates that we are able to outperform state-of-the-art algorithms on a variety of instances.

==> pics/combine_solution_offspring_LS_fm <==
% Just an ordinary comment
%
% A special comment:
% fmopt: width=6cm
%
% Another special comment:
% head:
% \usepackage{amsmath}
% end head

% psfrag commands:
\psfrag{A}{$V_1$}
\psfrag{C}{$S$}
\psfrag{B}{$V_2$}


==> pics/combine_solution_offspring_one_fm <==
% Just an ordinary comment
%
% A special comment:
% fmopt: width=6cm
%
% Another special comment:
% head:
% \usepackage{amsmath}
% end head

% psfrag commands:
\psfrag{A}{$V_1$}
\psfrag{C}{$S$}
\psfrag{B}{$V_2$}


==> pics/combine_solution_one_fm <==
% Just an ordinary comment
%
% A special comment:
% fmopt: width=6cm
%
% Another special comment:
% head:
% \usepackage{amsmath}
% end head

% psfrag commands:
\psfrag{A}{$V_1$}
\psfrag{C}{$S$}
\psfrag{B}{$V_2$}


==> pics/combine_solution_two_fm <==
% Just an ordinary comment
%
% A special comment:
% fmopt: width=6cm
%
% Another special comment:
% head:
% \usepackage{amsmath}
% end head

% psfrag commands:
\psfrag{A}{$V_1$}
\psfrag{C}{$S$}
\psfrag{B}{$V_2$}

